Efficient Self-supervised Vision Pretraining with Local Masked Reconstruction

Self-supervised learning for computer vision has achieved tremendous progress and improved many downstream vision tasks such as image classification, semantic segmentation, and object detection. Among these, generative self-supervised vision learning approaches such as MAE and BEiT show promising performance. However, their global masked reconstruction mechanism is computationally demanding. To address this issue, we propose local masked reconstruction (LoMaR), a simple yet effective approach that performs masked reconstruction within a small window of 7$\times$7 patches on a simple Transformer encoder, improving the trade-off between efficiency and accuracy compared to global masked reconstruction over the entire image. Extensive experiments show that LoMaR reaches 84.1% top-1 accuracy on ImageNet-1K classification, outperforming MAE by 0.5%. After finetuning the pretrained LoMaR on 384$\times$384 images, it can reach 85.4% top-1 accuracy, surpassing MAE by 0.6%. On MS COCO, LoMaR outperforms MAE by 0.5 $\text{AP}^\text{box}$ on object detection and 0.5 $\text{AP}^\text{mask}$ on instance segmentation. LoMaR is especially more computation-efficient on pretraining high-resolution images, e.g., it is 3.1$\times$ faster than MAE with 0.2% higher classification accuracy on pretraining 448$\times$448 images. This local masked reconstruction learning mechanism can be easily integrated into any other generative self-supervised learning approach. Our code is publicly available in https://github.com/junchen14/LoMaR.

==> figures/vis_2.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.94\linewidth]
                  {pictures/different-ratio.pdf}
\caption{Reconstruction examples of sampled ImageNet (upper two rows) and COCO (lower two rows) validation images under different masking ratios ranging from 60\% to 90\%.}
\label{mask_ratio_visualization}
\vspace{-2mm}
\end{figure*}


==> rebut.tex <==
\newcommand{\ReviewerA}{\textbf{\textcolor{cyan}{@R1}}}
\newcommand{\ReviewerB}{\textbf{\textcolor{magenta}{@R2}}}
\newcommand{\ReviewerC}{\textbf{\textcolor{blue}{@R3}}}




%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
\noindent We sincerely thank the reviewers for their thoughtful feedback. We are encouraged that all the reviewers \ReviewerA\ReviewerB\ReviewerC~agree that LoMaR is more efficient than the baselines. \ReviewerA \ReviewerB~LoMaR is more effective compared to prior work. We address below the reviewers’ comments and have incorporated all the feedback to enhance our work.

\noindent\ReviewerA: \textbf{LoMaR's windows may remove larger portions of an image. This is potentially a problem for classification if the image subject is not visible for "unlucky" input views.} During pre-training, the goal of LoMaR encoder is to learn robust representations. As shown in Fig.~\ref{reconstruction}, LoMaR can understand images through local reconstruction. This local sampling is applied during pre-training only and does not impact downstream tasks carried out after fine-tuning the encoder. After pre-training, LoMaR encoder is fine-tuned for various downstream tasks, following a process similar to MAE. Please note that neither LoMaR nor MAE employs masking during downstream tasks such as classification, segmentation, or object detection. \noindent\ReviewerA: \textbf{Why zero out the masked patches and not remove them from input sequence as in MAE?}  We feed the masked patches along with the unmasked ones into the encoder. We find that inputting the masks in the early stages can enhance the visual representation and make it more robust to mask reconstruction from the smaller regions, improving the performance of LoMaR. This could be because the encoder can convert the masked patches back to their original RGB representation after multiple encoder layers interact with the other visible patches. Those recovered masks in the hidden layers can implicitly contribute to the image representation. \ReviewerA: \textbf{ Why average over of all features of patches? Is the CLS token not used? Do the authors mean average over regions?}The CLS token is fed as input, but we take the average over all features of patches following the same practice as MAE. 
\ReviewerA: \textbf{Results for 300 epochs for MAE} At 300 epochs, MAE achieves an accuracy of 82.9\%, which is same as BEiT, while LoMaR achieves 83.3\%. \ReviewerA: \textbf{Why bold results for LoMaR In Table 2} This was done as we considered MAE and BEiT the main competitors. However, we agree this may not be the case, and we have updated the table accordingly. \ReviewerA: \textbf{For (DINO,...,SemMAE), perhaps separate these with a horizontal line} Thank you for your suggestion. We have updated the table. \ReviewerA: \textbf{Sec 4.2 also mentions Lomar at 1600 epochs but doesn't explain that this corresponds to the result in Figure 3 at roughly 250 hours.} From Table 2, it can be seen that LoMaR takes 66 hours for 400 epochs, so it takes 66 $\times$ 4(264) hours for 1,600 epochs. The primary purpose of Figure 3 is to compare the efficiency, while Table 2 shows the performance achieved. We have added the text in Sec 4.2 to comment on Figure 3. \ReviewerA: \textbf{Table 6 caption doesn't explain the purpose of the table.} Sorry for this. We have updated the caption to better reflect the table content. \ReviewerA: \textbf{Line 724:text makes it seem like the performance "does not change much" for all window sizes not only for 14x14 vs 7x7} We have updated the text to clarify that we want to convey that the performance change is low when going from 14 to 7 sizes window and not for all the sizes.   \ReviewerA: \textbf{Evaluations comparing other methods use LoMaR with RPE/APE? Is this fair for MAE/BEiT?} We use LoMaR with RPE for comparison, MAE uses APE, and BEiT uses RPE. We tried MAE with RPE but did not notice gains. From our experiments, RPE does not improve MAE; this could be because the entire image is used, and there may not be any benefit from RPE over APE. \ReviewerA: \textbf{Typos and inconsistency}. Thank you for the suggestions; we have updated the text.

\noindent \ReviewerB: \textbf{local reconstruction can limit model performance for long-range dependency.} We agree that local reconstruction can limit the model's ability to capture long-range dependencies. However, as shown in Fig.~\ref{fig:attention}, the reconstruction task in our experiments primarily focuses on local image regions, enabling the model to learn good representations effectively even with local reconstruction. Moreover, the pre-trained LoMaR encoder model can be fine-tuned for various downstream tasks, allowing it to learn more complex relationships, including long-range dependencies. Our empirical results show that LoMaR achieves competitive performance on various tasks. LoMaR's ability to learn good representations from local patches and its adaptability for downstream tasks are factors in its overall performance.


\noindent \ReviewerC: \textbf{lack of novelty}: Our method differs from cropping small images from high-resolution images. Taking MAE as an example, when it crops the image 448x448 into 384x384 regions, it still requires inputting a large number of patches as input (576 x 0.25 = 144 patches for MAE encoder input and 576 patches for MAE decoder input). However, LoMaR only takes (49 patches as input for both LoMaR encoder and decoder). This difference in the amount of input patches will significantly influence the training efficiency, especially for the high-resolution images. This is one of the most important novelty for improving the training efficiency compared to previous methods. The difference between our model architecture design is also essential for the model's performance. As shown in Figure 4, directly applying window-based masking to MAE, equivalent to cropping the images, does not work as well as LoMaR. This model architecture is also critical to achieving good performance compared to previous architectures such as MAE. \ReviewerC: \textbf{out of date baselines}: \href{https://link.springer.com/article/10.1007/s11263-023-01852-4}{Context Auto-Encoder}~\cite{ContextAutoencoder2022} published in IJCV, 2024 has been updated in the comparison. \ReviewerC: \textbf{ fairness of comparison} In Tables~\ref{high_resolution} and~\ref{imagenet_results}, all methods(including LoMaR) are trained on same resolution. Tables~\ref{object_detection} and~\ref{sementic_segmentation} show LoMaR performance on 224 and 384 resolutions. For classification and detection, LoMaR outperforms baselines while being trained on 224x224 images. \ReviewerC: \textbf{reproducibility}: We have attached the code.
% with supplementary.

%%%%%%%%% REFERENCES
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }


